Evaluating Fairness in Black-box Algorithmic Markets: A Case Study of Ride Sharing in Chicago

This study examines fairness within the rideshare industry, focusing on both drivers' wages and riders' trip fares. Through quantitative analysis, we found that drivers' hourly wages are significantly influenced by factors such as race/ethnicity, health insurance status, tenure to the platform, and working hours. Despite platforms' policies not intentionally embedding biases, disparities persist based on these characteristics. For ride fares, we propose a method to audit the pricing policy of a proprietary algorithm by replicating it; we conduct a hypothesis test to determine if the predicted rideshare fare is greater than the taxi fare, taking into account the approximation error in the replicated model. Challenges in accessing data and transparency hinder our ability to isolate discrimination from other factors, underscoring the need for collaboration with rideshare platforms and drivers to enhance fairness in algorithmic wage determination and pricing.

==> sections/_deprecated_2_related_work.tex <==
\section{Related Work}
% The literature review should address the following:
% \begin{enumerate}
%     \item the broad consensus and/or dissension in your topic
%     \item the open problem(s), if any
%     \item the gap in the literature that your project aims to fill
% \end{enumerate}
\subsection{Algorithmic Decision Making of Wages in Platform Economy}
Recent research has revealed that inequality exists between different genders, races, and socioeconomic statuses in the gig economy~\cite{hsieh2023designing}. This inequality contains many aspects, and one of the most important issues that attracted attention from workers is the pay gap. Preliminary studies have shown that the pay gap exists in crowdsourcing and freelancing platforms~\cite{dubey2017analyzing, dunn2021gender, foong2021understanding}. In such platforms, compensation often aligns with the standards set by service requesters~\cite{jarrahi2019algorithmic, jarrahi2020platformic}. In the rideshare industry, the situation is different: drivers' wages are determined by the platform algorithm. To understand the payment structure and identify fairness issues, Cook et al. conducted a quantitative analysis examining the gender pay gap in Uber drivers. In their study, they analyze the gender pay gap with race and experience controls, and their results show that similar to the traditional workforce, the wage gap exists in the rideshare industry~\cite{cook2021gender}. In our study, we separate these features and re-evaluate the fairness of the algorithm. Furthermore, we intend to explore other socioeconomic features closely related to drivers' work but haven't been examined in previous studies, such as health insurance coverage and the highest level of education received. We have run the analysis of these features as well. 


\subsection{Algorithmic Decision Making of Prices in Platform Economy}
The algorithmic decision not only determines the wage of drivers but also the price paid by riders. Unlike Taxi, which provides a similar transportation service but a more transparent and fixed pricing strategy, the price in ridesharing services is dynamic, impacted by trip distance, time, and the demand-supply status~\cite{shapiro2018between, pandit2019pricing, chen2015peeking}. Since most of the work in this field focuses on the well-being of the worker side, the other side of the market is often overlooked. Inspired by prior works \cite{ge2020racial, brown2018ridehail} revealing discrimination in ridsharing, such as unequal wait times and cancellation rates across different demographic groups, we aim to further explore unfairness from the customers' point of view and ask \textit{whether riders get fairly charged for the service they received.}

\subsection{Quantifying and Mitigating Fairness Disparities}
Many research literature addresses similar concerns related to our research questions across various datasets and aspects of the ridesharing economy. For example, in studies focusing on Uber and similar platforms, Ge et al. uncovered gender and racial biases towards customers \cite{ge2020racial}. Similarly, Brown examined potential biases in the frequency of rideshare service usage and equal accessibility in specific areas \cite{brown2018ridehail}. While these studies primarily explored biases from a customer perspective, our research aims to analyze fairness in both the pricing of rideshare services for riders and the compensation provided to drivers.

Beyond the rideshare industry, \cite{cohen2022price} investigated fairness in pricing strategies, highlighting the challenges in achieving satisfactory fairness constraints within pricing algorithms due to factors such as price, demand, and consumer surplus. Additionally, works by \cite{feldman2015certifying, zemel2013learning, mitchell2021algorithmic} offer frameworks and methodologies for quantifying and mitigating bias in datasets and prediction-based decision-making processes. For our project, we incorporate insights and methods from these works to analyze datasets specifically related to drivers and customers of rideshare platforms.  


==> sections/_deprecated_4_results.tex <==
\section{Results}
\subsection{Fairness in driver's compensation}
Based on our analysis, age and the highest level of education did not contribute to any notable difference in rideshare platform driver's hourly wage. However, the following features had a significant impact: race/ethnicity, health insurance status, driver’s tenure and weekly working hours. This conclusion was mainly based on the results of Chi-square tests with respect to each feature on driver's hourly wage. The specific differences in hourly wages among groups for each feature are detailed below.

For race and ethnicity, drivers who identified themselves as Asian/Asian American had the lowest median and mode hourly wage (both being \$12-13) among all race and ethnicity groups. The stacked bar graph (Figure \ref{fig:race}) showed that the distribution of hourly wage for Asian/Asian American drivers was skewed towards the lower wage categories compared to other groups, and the result of a pairwise Chi-square test further confirmed that this difference in wage distribution was statistically significant. 

For health insurance status, drivers with Medicaid/Medicare insurance received the lowest hourly wage in terms of median and mode (mean = \$12-13, mode = <\$10) compared to drivers with other types of insurance. The wage gap was especially large if we considered the mode hourly wage for each group given that the mode for all other groups was \$20+. Similarly, we observed that the distribution of hourly wage for drivers with Medicaid/Medicare insurance was skewed towards the lower wage categories compared to other groups (Figure \ref{fig:insurance}), and the result of a pairwise Chi-square test showed the statistical significance of such difference.

For driver's tenure, our results revealed that both drivers who stayed the shortest (less than 1 year) and the longest (10+ years) with the platform earned lower hourly wages. The mode hourly wage for these two groups was <\$10, and the median for both groups was \$12-13 (Figure \ref{fig:tenure}). Originally, we hypothesized that drivers who had been working with the platform for longer would be earning more, which would generally be true in many other industries. However, our analysis rejected the hypothesis. The result of a pairwise Chi-square test demonstrated that the hourly wage distribution for drivers who stayed the shortest and the longest with the platform was statistically significant from drivers who lay in the middle.

Lastly, for driver's weekly working hours, we found that drivers' hourly wage increased as their weekly working hours increased (Figure \ref{fig:working_hours}). Our initial hypothesis was that when drivers drive longer, their earnings won’t increase due to gamification in the gig economy mentioned in previous literature~\cite{nagarajrao2024navigating, woodcock2018gamification}. However, our analysis shows proof against this hypothesis since there was a positive correlation between working hours and wage, and a pairwise Chi-square test showed statistical significance among different groups. 

Additionally, by examining the coefficients of the linear regression model that took all features above as inputs, we observed that race/ethnicity had the strongest effect on hourly wage. The effect magnitude of health insurance status, driver’s tenure and weekly working hours were similar and ranked just below the effect of race/ethnicity.

\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=\linewidth]{figures/race.png}
\end{center}
\caption{
Distribution of race groups in each hourly wage category. }
\label{fig:race}
\end{figure}

\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=\linewidth]{figures/insurance.png}
\end{center}
\caption{
Distribution of insurance groups in each hourly wage category. }
\label{fig:insurance}
\end{figure}

\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=\linewidth]{figures/tenure.png}
\end{center}
\caption{
Distribution of hourly wage category for each tenure group. }
\label{fig:tenure}
\end{figure}

\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=\linewidth]{figures/weekly_hour.png}
\end{center}
\caption{
Distribution of hourly wage category for each working hour group. }
\label{fig:working_hours}
\end{figure}

\subsection{Fairness in customer's payment}
The linear regression model we used to replicate the pricing algorithm of the rideshare platform had an RMSE of 5.35 and a $R^2$ of 0.69 when tested with the holdout test data from the TNP dataset. The estimated coefficients for each input feature demonstrated that pick-up and drop-off locations, trip mileage, and trip duration had the most significant impact on trip fares. Fares increased by approximately \$3 to \$7 in community areas such as 76 and 56 compared to other areas. It is possible that the rideshare platforms were unfairly overcharging riders who commute to and from these areas. However, given that the TNP dataset did not provide demographics about each community area, and we could not control for confounding factors such as demand and supply in each area, these patterns can not directly prove that biases and discrimination existed in the pricing algorithm.

With the predicted trip fares generated by our model, we did not observe a trend where the predicted fares were consistently higher or lower than the actual fares. However, the scatter plot in Figure \ref{fig:actualvspredict} showed that only a small number of data points seemed to be on the red dotted line where the predicted and actual fares matched. The result of Mann–Whitney U test confirmed that there was a statistically significant difference between the distribution of predicted trip fares and actual taxi fares (rejected the $H_{0}$ hypothesis with $p \text{ value}=0.0$). Further analysis revealed that 42\% of the predicted fares were lower than actual taxi fares, while 58\% were higher. Therefore, based on the sole comparison of overall predicted fares and the actual taxi fares, riders could be either over-charged or under-charged based on specific characteristics of their trips. It is difficult to conclude whether the rideshare platforms were fairly charging the customers since the pricing could be highly dynamic based on the demand and supply at the time that trips were booked.


\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=\linewidth]{figures/predicted_vs_actual_fare.png}
\end{center}
\caption{
Comparison between the actual taxi fares and the predicted fares if trips were fulfilled by rideshare platforms. Each data point represents one trip. Points above the red dotted line indicate predicted fares are higher than actual fares, while points below indicate predicted fares are lower than actual fares.
}
\label{fig:actualvspredict}
\end{figure}
